Leveraging Traceability to Integrate Safety Analysis Artifacts into the Software Development Process

Safety-critical system's failure or malfunction can cause loss of human lives or damage to the physical environment; therefore, continuous safety assessment is crucial for such systems. In many domains this includes the use of Safety assurance cases (SACs) as a structured argument that the system is safe for use. SACs can be challenging to maintain during system evolution due to the disconnect between the safety analysis and system development process. Further, safety analysts often lack domain knowledge and tool support to evaluate the SAC. We propose a solution that leverages software traceability to connect relevant system artifacts to safety analysis models, and then uses these connections to visualize the change. We elicit design rationales for system changes to help safety stakeholders analyze the impact of system changes on safety. We present new traceability techniques for closer integration of the safety analysis and system development process, and illustrate the viability of our approach using examples from a cyber-physical system that deploys Unmanned Aerial Vehicles for emergency response.

==> sections/background.tex <==
\section{Safety Analysis Techniques \& Safety-Cases}
% The safety analysis process aims to evaluate the risks present in the system requirements and plan control measures when designing a safety-critical system. Safety-critical software products from domains such as Aviation, Railways, and Medical have extensively applied FTA and FMECA techniques to conduct the safety analysis. FTA is a top-down approach that starts with evaluating events that could cause a system-level failure and refines those events until the process determines the root causes of failure. FTA organizes the cause and effects of failure into a hierarchy of events connected by symbols depicting a  logical relation between them. FMECA is a bottom-up approach that starts with the investigation of component failures and seeks potential causes and effects of each failure. The FEMCA captures its results in a tabular structure. 

% The system design or implementation frequently changes due to factors such as optimizations, refactoring, or feature enhancements. Such changes could introduce new risks or faults in the system. The analysts need to analyze the deviation in system properties due to those changes and recognize its impact on safety. Such analysis requires extensive domain knowledge and technical expertise to accurately judge the impact of change (cite kelly paper here - internal source change). Therefore, there is a need for advanced tool support to guide stakeholders in analyzing changes. Fault Trees and FMECA reports contain multiple pieces of information such as (1) The root cause of risk, (2) The effect of risk on the system, and (3) Strategy to mitigate the risk. Safety analysts are expected to use their domain expertise to identify the association of system changes with some root causes and effects of risk. Failure in associating such a relationship results in inadequate confidence among stakeholders in the system's safety. 
% We believe that the abstraction of risk causality and consequence from safety analysis artifacts could assist in automatically generating the rationales for changes in different development artifacts. For example, a change in the design to optimize a feature could be justified as safe if that still addresses the same cause of risk and capable of preventing the system from the same risk effect. 


\subsection{SAFA Framework}

% The SAFA framework compares the current version of the system with a baseline version to graphically visualize the changes in artifacts such as requirements, design choices, code, operating context, and environmental assumptions. The delta visualization of artifacts guides the safety analysts to argue the impact of change over safety. The study with safety experts states that a significant number of users suggested adding the rationales behind the changes to assist them in critical thinking and change analysis. 
% Therefore, we intend to seek rationale behind the design changes and enforce them to argue that the change is safe.
% This paper aims at extending the SAFA framework by generating rationales from the elements of the safety analysis artifacts and allowing users to use those rationales in arguing the safety of the system. 




==> sections/conclusion.tex <==
\section{Conclusion}
In this paper,we present a novel solution to analyse the impact of system changes on the safety. We demonstrate the suitability of our solution by analysing the changes of an emergency response system. we further aim at extending the solution to make it adaptable in agile environment.

==> sections/proposal.tex <==
\section{Overview of the Proposed Approach}
\begin{figure}
    \centering
\includegraphics[width=\columnwidth]{images/Overview_new_simple.jpg}
    \caption{Caption \jch{We need to remove the risk thing from the middle, and redo the safety case so that it is more 'typical' and not SAFA style.  We can sketch quickly on my whiteboard after 10.30 (I have a 10.00am meeting)}  Ankit, please think about what the safety assurance case might look like if it were not SAFA style.  In other words it should definitely not be a hierarchy of artifacts).}
    \label{fig:fta}
\end{figure}


\section{Safety Case Change Analysis}
% Example and guiding questions would go here...

\subsection{Restricted Airspace Scenario}
\subsection{System Changes}
\subsection{Rationales}
\begin{figure}
    
    \includegraphics[width=0.5\columnwidth]{images/Restricted_airspace_FTA.jpg}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



==> sections/section_ConnectingToSACs.tex <==
\section{Connecting Safety Analysis Artifacts with SACs}
MOVED to Section on Safety
